TadGAN: Time Series Anomaly Detection Using Generative Adversarial Networks

Time series anomalies can offer information relevant to critical situations facing various fields, from finance and aerospace to the IT, security, and medical domains. However, detecting anomalies in time series data is particularly challenging due to the vague definition of anomalies and said data's frequent lack of labels and highly complex temporal correlations. Current state-of-the-art unsupervised machine learning methods for anomaly detection suffer from scalability and portability issues, and may have high false positive rates. In this paper, we propose TadGAN, an unsupervised anomaly detection approach built on Generative Adversarial Networks (GANs). To capture the temporal correlations of time series distributions, we use LSTM Recurrent Neural Networks as base models for Generators and Critics. TadGAN is trained with cycle consistency loss to allow for effective time-series data reconstruction. We further propose several novel methods to compute reconstruction errors, as well as different approaches to combine reconstruction errors and Critic outputs to compute anomaly scores. To demonstrate the performance and generalizability of our approach, we test several anomaly scoring techniques and report the best-suited one. We compare our approach to 8 baseline anomaly detection methods on 11 datasets from multiple reputable sources such as NASA, Yahoo, Numenta, Amazon, and Twitter. The results show that our approach can effectively detect anomalies and outperform baseline methods in most cases (6 out of 11). Notably, our method has the highest averaged F1 score across all the datasets. Our code is open source and is available as a benchmarking tool.

==> tables/baseline_point.tex <==
\begin{center}
  \begin{table*}
  \caption{F1-Scores of baseline models using point-wise identification method.}
  \begin{tabulary}{1.5\textwidth}{LLLLLLLLLLLL}
  \toprule
   & \multicolumn{11}{c}{\textbf{Data sets}} \\
  %  \hline
   & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
    \cmidrule(r){2-3}\cmidrule(r){4-7}\cmidrule(r){8-12}
  \textbf{Baseline} & MSL & SMAP & A1 & A2 & A3 & A4 & Art & AdEx & AWS & Traf & Tweets\\
  \toprule
  \name  
  &\textbf{0.623} & \textbf{0.704}
  & \textbf{0.8} & 0.862 & 0.685 & 0.599
  & \textbf{0.909} & \textbf{0.8} & 0.644 & 0.486 & \textbf{0.59} \\
  \hline
  HTM      
  & {\cellcolor{c4}}0.43  & {\cellcolor{c5}}0.536 
  & {\cellcolor{c6}}0.605 & {\cellcolor{c6}}0.653 & {\cellcolor{c3}}0.331 & {\cellcolor{c2}}0.29  
  & {\cellcolor{c4}}0.455 & {\cellcolor{c5}}0.552 & {\cellcolor{c6}}0.6   & {\cellcolor{c4}}0.474 & {\cellcolor{c5}}0.508\\
  Arima   
  & {\cellcolor{c4}}0.492 & {\cellcolor{c4}}0.42  
  & {\cellcolor{c7}}0.726 & {\cellcolor{c8}}0.836 & {\cellcolor{c8}}0.815 & {\cellcolor{c7}}0.703 
  & {\cellcolor{c3}}0.353 & {\cellcolor{c5}}0.583 & {\cellcolor{c5}}0.518 & {\cellcolor{c5}}0.571 & {\cellcolor{c5}}0.567\\
  LSTM   
  & {\cellcolor{c4}}0.46  & {\cellcolor{c6}}0.69  
  & {\cellcolor{c7}}0.744 & {\cellcolor{c9}}\textbf{0.98}  & {\cellcolor{c7}}0.772 & {\cellcolor{c6}}0.645
  & {\cellcolor{c3}}0.375 & {\cellcolor{c5}}0.538 & {\cellcolor{c4}}0.474 & {\cellcolor{c6}}\textbf{0.634} & {\cellcolor{c5}}0.543\\
  Dense AE 
  & {\cellcolor{c5}}0.507 & {\cellcolor{c7}}0.7  
  & {\cellcolor{c4}}0.472 & {\cellcolor{c2}}0.294 & {\cellcolor{c0}}0.074 & {\cellcolor{c0}}0.09  
  & {\cellcolor{c4}}0.444 & {\cellcolor{c2}}0.267 & {\cellcolor{c6}}0.64  & {\cellcolor{c3}}0.333 & {\cellcolor{c0}}0.057\\
  LSTM AE 
  & {\cellcolor{c5}}0.507 & {\cellcolor{c6}}0.672 
  & {\cellcolor{c6}}0.608 & {\cellcolor{c8}}0.871 & {\cellcolor{c2}}0.248 & {\cellcolor{c1}}0.163 
  & {\cellcolor{c5}}0.545 & {\cellcolor{c5}}0.571 & {\cellcolor{c7}}\textbf{0.764} & {\cellcolor{c5}}0.552 & {\cellcolor{c5}}0.542\\
  MAD-GAN   
  & {\cellcolor{c1}}0.154 & {\cellcolor{c1}}0.14  
  & {\cellcolor{c2}}0.244 & {\cellcolor{c2}}0.205 & {\cellcolor{c0}}0.056 & {\cellcolor{c0}}0.096 
  & {\cellcolor{c1}}0.153 & {\cellcolor{c3}}0.308 & {\cellcolor{c1}}0.136 & {\cellcolor{c1}0.1   & {\cellcolor{c2}}0.237\\
  MS Azure  
  & {\cellcolor{c2}}0.218 & {\cellcolor{c1}}0.118 
  & {\cellcolor{c3}}0.352 & {\cellcolor{c6}}0.612 & {\cellcolor{c2}}0.257 & {\cellcolor{c2}}0.204 
  & {\cellcolor{c1}}0.125 & {\cellcolor{c0}}0.066 & {\cellcolor{c1}}0.173 & {\cellcolor{c1}}0.166 & {\cellcolor{c1}}0.118\\
  \toprule
  \end{tabulary}
  \label{tab:Baselines}
  \end{table*}
\end{center}

==> tables/variation1.tex <==
% \begin{center}
%   \begin{table*}
%   \caption{F1-Scores of different variations of our model.}
%  %  \tiny
%   %\begin{tabulary}{\textwidth}{p{1.2cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}}
%   \begin{tabulary}{1.5\textwidth}{LLLLLLLLLLLL}
%   \toprule
%   %  \hline
%   & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
%     \cmidrule(r){2-3}\cmidrule(r){4-7}\cmidrule(r){8-12}
%   \textbf{Variation} 
%   & MSL & SMAP 
%   & A1 & A2 & A3 & A4 
%   & Art & AdEx & AWS & Traf & Tweets\\
%   \toprule
%   Critic       
%   & 0.393  & 0.672 
%   & 0.285  & 0.118  & 0.008  & 0.024
%   & \textbf{0.909} & 0     & 0.35  & 0.167 & 0.548 \\
%   Point        
%   & 0.585  & 0.588 
%   & 0.674  & 0.806 & 0.628 & \textbf{0.599 }
%   & 0.588  & 0.611 & 0.551 & 0.383 & 0.571 \\
%   Area         
%   & 0.525 & 0.655 
%   & 0.681  & 0.735 & 0.567 & 0.523
%   & 0.625 & 0.645 & 0.59  & 0.435 & 0.559 \\
%   DTW          
%   & 0.514 & 0.581 
%   & 0.697  & \textbf{0.862} & 0.613 & 0.547 
%   & 0.714 & 0.69   & 0.633 & 0.455 & 0.559 \\
  
%   Critic$\times$Point 
%   & 0.619 & 0.675 
%   & 0.703  & 0.678  & \textbf{0.685} & 0.536
%   & 0.588 & 0.579  & 0.576 & 0.4 & 0.59 \\
%   Critic$\times$Area  
%   & 0.578 & \textbf{0.704} 
%   & 0.719 & 0.701 & 0.587 & 0.46
%   & 0.8    & 0.6  & 0.6 & 0.4 & 0.571 \\
%   Critic$\times$DTW   
%   & \textbf{0.623} & 0.68  
%   & 0.667 & 0.727 & 0.631 & 0.497
%   & 0.667 & 0.667 & 0.61 & 0.455 & 0.605 \\
  
%   Critic+Point 
%   & 0.529 & 0.653
%   & \textbf{0.8}  & 0.727  & 0.571  & 0.44
%   & 0.625 & 0.595  & \textbf{0.644} & 0.439 & 0.592 \\
%   Critic+Area  
%   & 0.493 & 0.692
%   & 0.789 & 0.745 & 0.483 & 0.367
%   & 0.75  & 0.75  & 0.607 & 0.474 & 0.6 \\
%   Critic+DTW   
%   & 0.462 & 0.658  
%   & 0.735 & 0.807 & 0.523 & 0.388
%   & 0.667 & \textbf{0.8}  & 0.632 & \textbf{0.486} & \textbf{0.609} \\
%   \toprule
%   \end{tabulary}
%   \label{tab:evaluation}
%   \end{table*}
% \end{center}

\begin{center}
  \begin{table*}[t]
   \caption{F1-Scores of the variations of our model that only use \textit{Critic} outputs or reconstruction errors.}
 %  \tiny
  %\begin{tabulary}{\textwidth}{p{1.2cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}}
  \begin{tabulary}{1.5\textwidth}{LLLLLLLLLLLL}
  \toprule
  %  \hline
   & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
    \cmidrule(r){2-3}\cmidrule(r){4-7}\cmidrule(r){8-12}
  \textbf{Variation} 
  & MSL & SMAP 
  & A1 & A2 & A3 & A4 
  & Art & AdEx & AWS & Traf & Tweets\\
  \toprule
  Critic       
  & 0.393  & \textbf{0.672 }
  & 0.285  & 0.118  & 0.008  & 0.024
  & 0.625 & 0     & 0.35  & 0.167 & 0.548 \\
  Point        
  & \textbf{0.585}  & 0.588 
  & 0.674  & 0.758 & \textbf{0.628} & \textbf{0.599 }
  & 0.588  & 0.611 & 0.551 & 0.383 & 0.571 \\
  Area         
  & 0.525 & 0.655 
  & 0.681  & \textbf{0.82} & 0.567 & 0.523
  & 0.625 & 0.645 & 0.59  & 0.435 & \textbf{0.559} \\
  DTW          
  & 0.514 & 0.581 
  & \textbf{0.697}  & 0.794 & 0.613 & 0.547 
  & \textbf{0.714} & \textbf{0.69}   & \textbf{0.633} & \textbf{0.455} & \textbf{0.559} \\
  
  \toprule
  \end{tabulary}
  \label{tab:evaluation1}
  \end{table*}
\end{center}



==> tables/variation2.tex <==

\begin{center}
  \begin{table*}[t]
   \caption{F1-Scores of the variations of our model that combine \textit{Critic} outputs and reconstruction errors. The top row ``Best Single'' reports the best F1 scores from Table~\ref{tab:evaluation1}}
 %  \tiny
  %\begin{tabulary}{\textwidth}{p{1.2cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}p{0.4cm}}
  \begin{tabulary}{1.5\textwidth}{LLLLLLLLLLLL}
  \toprule
  %  \hline
   & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
    \cmidrule(r){2-3}\cmidrule(r){4-7}\cmidrule(r){8-12}
  \textbf{Variation} 
  & MSL & SMAP 
  & A1 & A2 & A3 & A4 
  & Art & AdEx & AWS & Traf & Tweets\\
  \toprule
  Best Single   
  & 0.585  & 0.672 
  & 0.697  & 0.82  & 0.628  & \textbf{0.599}
  & 0.714 & 0.69   & 0.633  & 0.455 & 0.559 \\
  
  \hline
  Critic$\times$Point 
  & 0.619 & 0.675 
  & 0.703  & 0.75  & \textbf{0.685} & 0.536
  & 0.588 & 0.579  & 0.576 & 0.4 & 0.59 \\
  Critic$\times$Area  
  & 0.578 & \textbf{0.704} 
  & 0.719 & \textbf{0.867} & 0.587 & 0.46
  & \textbf{0.8}    & 0.6  & 0.6 & 0.4 & 0.571 \\
  Critic$\times$DTW   
  & \textbf{0.623} & 0.68  
  & 0.667 & 0.82 & 0.631 & 0.497
  & 0.667 & 0.667 & 0.61 & 0.455 & 0.605 \\
  
  Critic+Point 
  & 0.529 & 0.653
  & \textbf{0.8}  & 0.78  & 0.571  & 0.44
  & 0.625 & 0.595  & \textbf{0.644} & 0.439 & 0.592 \\
  Critic+Area  
  & 0.493 & 0.692
  & 0.789 & 0.847 & 0.483 & 0.367
  & 0.75  & 0.75  & 0.607 & 0.474 & 0.6 \\
  Critic+DTW   
  & 0.462 & 0.658  
  & 0.735 & 0.857 & 0.523 & 0.388
  & 0.667 & \textbf{0.8}  & 0.632 & \textbf{0.486} & \textbf{0.609} \\
  \toprule
  \end{tabulary}
  \label{tab:evaluation2}
  \end{table*}
\end{center}


==> texfiles/problem.tex <==
\section{Problem formulation}
\label{sec:problem}

Consider a time series $\mathbf{X}=(x^1, x^2, \cdots, x^T)$,  where $x^i \in \mathbf{R}^{M \times 1}$ indicates $M$ types of measurements at time step $i$.
The goal of time series anomaly detection is to find out a set of anomalous time segments $\bm{A_{seq}}=\{\bm{a_{seq}^1}, \bm{a_{seq}^2}, \cdots, \bm{a_{seq}^k}\}$, where $\bm{a_{seq}^i}$ is a continuous sequence of time steps that shows unusual behaviors (Figure~\ref{fig:anomaly_detection}). 
The ``unusual'' simply refers to the values of that segment appear to be extremely high/low or not comply with the expected temporal changes. 

We highlight that the length of $\bm{a^i}$ is variant. 
Compared with the time series classification problem where the length of the time segment is fixed, our problem thereby becomes much challenging.

Besides, given the fact that labeled data are not available for most real-world applications, in this work we only consider unsupervised solutions. 
Unlike supervised learning, unsupervised models do not train to optimize finding any ``known anomalies''. Rather, one trains to learn the time series patterns, detect anomalies and then check if the detector identified any ``known anomalies''. 

The known anomalies are the time segments that have been manually annotated as anomalies by human experts. Several datasets with their corresponding ``known anomalies'' exist, the details of which are introduced in Section~\ref{sec:datasets}. In this work, we leverage these ``known anomalies'' to evaluate the efficacy of our proposed unsupervised model and the details can be found in Section~\ref{sec:metrics}.



